An Analysis of Complex-Valued CNNs for RF Data-Driven Wireless Device Classification

Recent deep neural network-based device classification studies show that complex-valued neural networks (CVNNs) yield higher classification accuracy than real-valued neural networks (RVNNs). Although this improvement is (intuitively) attributed to the complex nature of the input RF data (i.e., IQ symbols), no prior work has taken a closer look into analyzing such a trend in the context of wireless device identification. Our study provides a deeper understanding of this trend using real LoRa and WiFi RF datasets. We perform a deep dive into understanding the impact of (i) the input representation/type and (ii) the architectural layer of the neural network. For the input representation, we considered the IQ as well as the polar coordinates both partially and fully. For the architectural layer, we considered a series of ablation experiments that eliminate parts of the CVNN components. Our results show that CVNNs consistently outperform RVNNs counterpart in the various scenarios mentioned above, indicating that CVNNs are able to make better use of the joint information provided via the in-phase (I) and quadrature (Q) components of the signal.

==> 04.NNArch_long.tex <==
% --------------------------------------

We now describe our experimental methodology, which includes details on the datasets used, the neural network architectures and the experiments conducted.

% --------------------------------------
\subsection{Dataset Construction for Experimental Evaluation} \label{sec:dc}
Evaluating machine learning algorithms involves evaluating how well a trained model (like our neural networks) generalize to an independent test set. Typically, an evaluation methodology like averaging over multiple random train/test splits or cross-validation is used. 
However, RF data experiences changes in the data distribution over the duration of the transmission. This non-stationary behavior violates the assumptions of standard machine learning evaluation methodologies. Data from different transmissions from the same device can also exhibit quite a large variance. As a result, we need to create a specialized evaluation methodology suitable for our RF data-based experiments.

Figure \ref{fig:ds_split} illustrates our evaluation methodology. In our dataset, there are $K$ devices (also corresponding to the number of classes) and $M$ transmissions per device. To mitigate the non-stationary behavior, we ensure that the training data is close in time to the test data. In addition, for a given device, we restrict the training and test data to be from the same transmission. We create a series of train/test partitions of the data, which we refer to as \emph{splits}. These splits are created over evenly-spaced time intervals over the transmission data as shown in Figure \ref{fig:ds_split}. 


% we report results averaged over $S\times K$ splits of the data, with each split containing a training and test partition of the data. However, due to rapid changes in the distribution of RF data during a transmission, we chose to create splits that keep the training data close in time to the test data. Figure (\ref{fig:ds_split}) illustrates the process.

\begin{figure}[ht]
  \centering \includegraphics[width=0.45\textwidth]{ds_split.pdf}
  \caption{Datasets Construction} % (Source: \cite{Trabelsi2018DeepCN})}
  \label{fig:ds_split}
\end{figure}

%
%Complicating this process is the fact that there are $K$ devices (also the number of classes) and $M$ transmissions per device. 
Due to data variability from one transmission to another, we create train-test datasets using data from the same transmission; in effect, this creates a set of split-transmission pairs. We create $S$ splits per transmission over all devices, with each split created at regular intervals as shown in Figure \ref{fig:ds_split}. 

To create each split, we first take the transmission data and divide it into thirds. We create the splits using the middle third of the data to avoid dealing with specialized data in the first or last third  of the transmission. Each split contains $1200$ consecutive IQ samples. We space these splits evenly throughout the middle third of the transmission. For each split, we create $1200$ overlapping sliding windows, where we refer to the data within a window as a \emph{slice}. Thus, using the first IQ sample of the split as the starting point, we take a window of $100$ samples as the first slice for a given device. Then, we advance the sliding window by a stride of size $1$ and take the next $100$ samples as the second slice. This process continues until the last sample of the split (as the starting point of the last slice). We repeat this process for each device. Each split-transmission dataset is formed by taking the union of the generated slices from split index $s$ from transmission $m$ over all devices. We report the average accuracy over the $S \times M$ splits. 
%
The total number of splits per device is $S \times M$. For \dsosu~datasets $K=25, M=1, S=50$ and for \dsne~datasets $K=20, M=3, S=50$.

We apply this methodology to construct datasets for each of the four studied dataset scenarios: \dsone{}, \dstwo{}, \stthree{}, and \stfour{}, with
\begin{enumerate}
    \item $50$ datasets constructed from LoRa Indoor scenario (\dsone{})
    \item $50$ datasets constructed from LoRa Outdoor scenario (\dstwo{}) 
    \item $150$ datasets constructed from setup 3 (wired) of the Northeastern dataset (\stthree{})
    \item $150$ datasets constructed from setup 4 (wireless) of the Northeastern dataset (\stfour{})
\end{enumerate} 
Each dataset has $1200\times K$ slices and each slice has a dimension of $2\times 100$. The ratio of training to testing instances is $5:1$ and we ensure that the training data has an equal number of slices from each device. The final results of our experiments evaluate and show the accuracy averaged over all splits in each datasets scenario.



% --------------------------------------
\subsection{Complex-Valued Neural Networks: CVNNs}
Early work on CVNNs used pure complex number operations and focused on the
topics of complex activation functions \cite{Nitta1997AnEO,Georgiou1992ComplexDB} and complex backpropagation \cite{Leung1991TheCB, Benvenuto1992OnTC}; this work was primarily intended for shallow neural networks. Modern software packages for deep networks are largely built around automatic differentiation for real values. Software to extend automatic differentiation to complex values is not currently mature and often suffers from numerical instability. As a result, modern software packages attempt to reuse real-valued functionality to approximate complex-valued building blocks such as complex-valued convolutional layer, complex-valued ReLUs, and complex-valued batch normalization layer \cite{Trabelsi2018DeepCN}. Other works \cite{Wolter2018ComplexGR,Yang2020ComplexTA} have extended these complex-valued building blocks to recurrent neural networks with gated and transformer features.

The most important component of CVNN is the complex-valued convolutional layer
which reflects the essential difference between the CVNNs and RVNNs. For the
complex-valued convolutional block with complex filter matrix $W = A + iB$ and
input vector $h = x + iy$; here, $A$ and $B$ are real matrices while $x$ and $y$ are
real vectors. The complex convolution can be expanded according the
distributive property of convolution operator:
\begin{equation}
  \label{eq:ccov1}
  \mathbf{W} * \mathbf{h}=(\mathbf{A} * \mathbf{x}-\mathbf{B} *
  \mathbf{y})+i(\mathbf{B} * \mathbf{x}+\mathbf{A} * \mathbf{y})
\end{equation}
We can rewrite the above equation to matrix form as:
\begin{equation}
  \label{eq:ccov2}
  \left[\begin{array}{c}{\operatorname{Re}(\mathbf{W} * \mathbf{h})} \\ {\operatorname{Im}(\mathbf{W} * \mathbf{h})}\end{array}\right]
  = \left[\begin{array}{rr}{\mathbf{A}} & {-\mathbf{B}} \\ {\mathbf{B}} & {\mathbf{A}}\end{array}\right]
  * \left[\begin{array}{l}{\mathbf{x}} \\ {\mathbf{y}}\end{array}\right]
\end{equation}
Equation \eqref{eq:ccov1} shows that the complex-valued convolutional layer needs two
real-valued convolutional filters $A$ and $B$. For the complex-valued vector $h$ with real part $x$ and imaginary part $y$, both the real and imaginary part of the output of complex-valued convolution operator consist of these four components ($A, B, x, y$). The only difference is, the real part of the output is the subtraction between $\mathbf{A} * \mathbf{x}$ and $\mathbf{B} * \mathbf{y}$, and the imaginary part is the addition between the cross terms $\mathbf{B} * \mathbf{x}$ and $\mathbf{A} * \mathbf{y}$. This interleaving between the real and imaginary components is the most significant difference between CVNNs and RVNNs.
  
%The real and imaginary parts of the complex number of output can be obtained by the addition and subtraction of convolution operators between the real and imaginary parts of the complex-valued convolutional filters and the complex number inputs. 



% --------------------------------------
\subsection{Neural Network Architectures} \label{sec:expr_nets}

Figure \ref{fig:rvnn5} and \ref{fig:cvnn5} show the architecture of the RVNN and
CVNN used in our experiments. To simplify the analysis, we used RVNNs and CVNNs with two convolutional layers; deeper networks would likely improve performance but at the cost of making the analysis much more complex. More specifically, the baseline RVNN has two real-valued convolutional layers (conv layers), with each conv layer followed by a batch normalization layer and a ReLU layer. The output of the second conv layer goes to an average pooling layer, which produces the output. We use a cross entropy loss function to train the network.

Conceptually, the CVNN has an analogous structure as the RVNN, except each layer now consists of a real-valued part and a complex-valued part. The details of both architectures can be found in Table \ref{tab:expr_arch}.
% The first conv layer has a filter size of $(1, 25)$ and stride size of $(1,
% 3)$, and its input and output volume are $[1\times 2\times 100]$ and
% $[128\times 2\times 26]$ respectively. The output volume of second conv layer
% is $[N_{class}\times 2\times 3]$.

%%%%%% separate version
% \begin{figure}[ht]
%   \centering \includegraphics[width=0.45\textwidth]{net_rvnn5.pdf}
%   \caption{Architecture of RVNN}% (Source: \cite{Trabelsi2018DeepCN})}
%   \label{fig:rvnn5}
% \end{figure}

% \begin{figure}[ht]
%   \centering \includegraphics[width=0.45\textwidth]{net_cvnn5.pdf}
%   \caption{Architecture of CVNN}% (Source: \cite{Trabelsi2018DeepCN})}
%   \label{fig:cvnn5}
% \end{figure}

%%%%%% merge version
\begin{figure}[ht]
  \centering 
  \subfloat[RVNN]{%
    \includegraphics[width=0.45\textwidth]{net_rvnn5.pdf}
    \label{fig:rvnn5}} 
  \quad 
  \subfloat[CVNN]{%
    \includegraphics[width=0.45\textwidth]{net_cvnn5.pdf}
    \label{fig:cvnn5}} 
  %
  \caption{Architecture of RVNN and CVNN}
  \label{fig:net_rvnn_cvnn}
  \end{figure}


\begin{table*}
  \caption{Details of the RVNN and CVNN architectures}
  \label{tab:expr_arch}
  \centering
  \begin{tabular}{@{}lll|lll@{}}
    \toprule
    \multicolumn{3}{l|}{\thead{RVNN (Real-Valued CNN)}} & \multicolumn{3}{l}{\thead{CVNN (Complex-Valued CNN)}}                               \\
    \toprule
    Layer Type           & Output Size            & Filter / Stride Size & Layer Type & Output Size                    & Filter / Stride Size \\
    \midrule
    Input                & $1\times 2\times 100$  &                  & Input      & $ 2 \times 1\times 1\times 100$ &                         \\
    Conv2D               & $128\times 2\times 26$ & (1, 25) / (1, 3) & CConv2D    & $ 2 \times 64\times 1\times 26$ & (1, 25) / (1, 3)        \\
    BatchNorm            & $128\times 2\times 26$ &                  & CBatchNorm & $2 \times 64\times 1\times 26$ &                          \\
    ReLU                 & $128\times 2\times 26$ &                  & CReLU      & $2 \times 64\times 1\times 26$ &                          \\
    Conv2D               & $20\times 2\times 3$   & (1, 20) / (1, 3) & CConv2D    & $2 \times 20\times 1\times 3$  & (1, 20) / (1, 3)         \\
    BatchNorm            & $20\times 2\times 3$   &                  & CBatchNorm & $2 \times 20\times 1\times 3$  &                          \\
    ReLU                 & $20\times 2\times 3$   &                  & CReLU      & $2 \times 20\times 1\times 3$  &                          \\
    AvgPool2D            & $20$                   & (2, 3) / (1, 1)  & CAvgPool2D & $2\times 20$                   & (1, 3) / (1, 1)          \\
    Cross Entropy of $x$ &                        &                  & Cross Entropy of $|z|$ &                                &              \\

    \bottomrule
  \end{tabular}
\end{table*}

It is challenging to perform a head-to-head comparison between a RVNN and an "equivalent" CVNN.
To establish an approximate form of equivalence, we keep the number of parameters for both types of neural networks equal to each other. 
%The majority of the parameters come from the two convolution layers. Since there is a batch normalization layer after conv layer, the bias parameter can be ignored. 
For instance, with the \stthree~datasets, both the RVNN and the CVNN have a total of 54400 parameters. We acknowledge that having an equal number of parameters is not exactly an "apples-to-apples" comparison as there are other architectural differences; consequently, we include additional experiments (e.g. experiments that change the input features and ablation experiments) to shed light on the capabilities of CVNNs over RVNNs.

%there are $20$ devices, and the (input, output) channel number of the first and second conv layer of RVNN is (1, 128) and (128, 20) specifically, and of CVNN is (1, 64) and (64, 20). Considering the filter size of each layer (see Table \ref{tab:expr_arch}), the total amount of the parameters in RVNN and CVNN is both 54400.

%%%%%% table for parameters
% Table \ref{tab:expr_param} provides a detailed description of the number of parameters in each convolutional layer.
% \begin{table*}
%   \caption{Parameter counting of RVNN and CVNN, $N_{class}=20$}
%   \label{tab:expr_param}
%   \centering
%   \begin{tabular}{@{}l|l|l@{}}
%     \toprule
%     & {\thead{RVNN}}                                   & {\thead{CVNN}}                                                                    \\
%     \midrule
%     \#Params of Conv1 / CConv1 & $ (1 \times 25 \times 1 + 0) \times 128 = 3200 $ & $ (1 \times 25 \times 1 + 0) \times 64 \times 2 = 3200 $     \\
%     \#Params of Conv2 / CConv2 & $ (1 \times 20 \times 128 + 0) \times 20 = 51200 $ & $ (1 \times 20 \times 64 + 0) \times 20 \times 2 = 51200 $ \\
%     \midrule
%     Total & $54400$                                          & $54400$                                                                           \\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% --------------------------------------
\subsection{Ablation Strategies} \label{sec:expr_ab}
%%%%%% separate version
% \begin{figure}[ht]
%   \centering \includegraphics[width=0.45\textwidth]{cf_rvnn2.pdf}
%   \caption{Computational Flow of RVNN} % (Source: \cite{Trabelsi2018DeepCN})}
%   \label{fig:cf_rvnn}
% \end{figure}

% \begin{figure}[ht]
%   \centering \includegraphics[width=0.45\textwidth]{cf_cvnn2.pdf}
%   \caption{Computational Flow of CVNN.} % (Source: \cite{Trabelsi2018DeepCN})}
%   \label{fig:cf_cvnn}
% \end{figure}
 
%%%%%% merge version
\begin{figure}[ht]
  \centering 
  \subfloat[RVNN]{%
    \includegraphics[width=0.45\textwidth]{cf_rvnn2.pdf}
    \label{fig:cf_rvnn}} 
  \quad 
  \subfloat[CVNN]{%
    \includegraphics[width=0.45\textwidth]{cf_cvnn2.pdf}
    \label{fig:cf_cvnn}} 
  %
  \caption{A schematic of the computational flow through a RVNN and a CVNN. \wkw{Need to label the top part of the CVNN as "real" and bottom as "imaginary"} \cj{how about this}}
  \label{fig:cf_rvnn_cvnn}
  \end{figure}

%%%%%% ablation viz on cf
% \begin{figure}[ht]
%   \centering \includegraphics[width=0.45\textwidth]{cf_ab12_out.pdf}
%   \caption{Computational Flow of
%     AB12-Out} % (Source: \cite{Trabelsi2018DeepCN})}
%   \label{fig:cf_ab12_out}
% \end{figure}

% \begin{figure}[ht]
%   \centering \includegraphics[width=0.45\textwidth]{cf_ab12_conv.pdf}
%   \caption{Computational Flow of
%     AB12-Conv} % (Source: \cite{Trabelsi2018DeepCN})}
%   \label{fig:cf_ab12_conv}
% \end{figure}
The main difference between the CVNN and the RVNN is due to the cross terms
between the real and imaginary parts in the multiplication and convolution
operations. Figures \ref{fig:cf_rvnn} and \ref{fig:cf_cvnn} illustrate the computational flow for a RVNN and a CVNN; the computational flow of a CVNN is much more complex than that of a RVNN. As a concrete example, take the first complex-valued convolutional layer ($1^{st}$ CConv Layer) and its associated Output ($1^{st}$ Output) in Figure \ref{fig:cf_cvnn}. The real part of the $1^{st}$ Output (orange blocks) comes from the linear combination of I data scanned by real filters and Q data scanned by imaginary filters (as shown by the grey arrows pointing to the $\ominus$), while the imaginary part of the $1^{st}$ Output (green blocks) comes from the cross terms formed by the linear combination of I data scanned by imaginary filters and Q data scanned by real filters (as shown by the gray arrows pointing to $\oplus$. Here the $\ominus$ and $\oplus$ symbols in Figure \ref{fig:cf_cvnn} correspond to the real ($\mathbf{A} * \mathbf{x}-\mathbf{B} *
\mathbf{y}$) and imaginary parts ($\mathbf{B} * \mathbf{x}+\mathbf{A} * \mathbf{y}$) of Equation \ref{eq:ccov1}.

We perform a deeper dive into the differences between the two models through a series of ablation experiments which remove parts of the CVNN, specifically parts that correspond to some of the cross terms. By "remove" we mean that we zero out the ablated component. If performance degrades significantly, then the portion of the CVNN that is removed is an important
component of the model. Figure \ref{fig:cf_cvnn} illustrates the CVNN as 2 layers, with each layer consisting of convolutional filters and an output. There is a set of 12 ablation experiments that can be defined by the following dimensions and values:
\begin{enumerate}
\item The layer to ablate: $1^{st}$ layer ({\bf L1}), $2^{nd}$ layer ({\bf L2}), or both ({\bf L12}) 
% \item The layer to ablate: $1^{st}$ layer ({\bf AB1}), $2^{nd}$ layer ({\bf AB2}), or both ({\bf AB12}) 
\item The component of the layer to ablate: the convolutional filter ({\bf C}) or the output ({\bf O}) 
\item The part of the component to keep: the real part ({\bf RE}) or the imaginary part ({\bf IM}) 

\end{enumerate}


  % \item To ablate different layers of CVNN. In our case, it is to ablate the
  %   first layer (AB1), second layer (AB2) or both (AB12)
  % \item To ablate different components of each convolutional layer. That is to
  %   ablate the output of the layer (AB-Out), or the convolutional filters of
  %   layer (AB-Conv) (see the difference between Figure \ref{fig:cf_ab12_out}
  %   and \ref{fig:cf_ab12_conv})

Table \ref{tab:expr_abs} summarizes the 12 ablation experiments, with the name of the experiment stated in each table cell. The naming convention follows the boldface labels chosen for each ablation dimension, concatenated with an underscore. For example, "L1\_O\_IM" ablates the $1^{st}$ Output and remove the imaginary part of the output (green blocks of the $1^{st}$ Output in Figure \ref{fig:cf_cvnn}). In our results, we only show results of the "IM" ablations which remove the imaginary part (of the output or convolutional filter) and keep the real part; the results of the "RE" ablations have equivalent performance.

\begin{table*}
  \caption{Ablation Models}
  \label{tab:expr_abs}
  \centering
  \begin{tabular}{@{}l|ll|ll@{}}
    \toprule
    \multicolumn{1}{l|}{\thead{}} & \multicolumn{2}{l|}{\thead{Ablate Outputs}} & \multicolumn{2}{l}{\thead{Ablate Conv Filters}} \\

    \toprule
                                  & Remove Re Output & Remove Im Output & Remove Re Conv   & Remove Im Conv                                                    \\

    \midrule
    L1 (Ablate $1^{st}$ Layer) & L1\_O\_RE  & \textbf{L1\_O\_IM}  & L1\_C\_RE & \textbf{L1\_C\_IM}                                                  \\
    L2 (Ablate $2^{nd}$ Layer) & L2\_O\_RE  & \textbf{L2\_O\_IM}  & L2\_C\_RE & \textbf{L2\_C\_IM}                                                  \\
    L12 (Ablate Both)          & L12\_O\_RE & \textbf{L12\_O\_IM} & L12\_C\_RE & \textbf{L12\_C\_IM}                                                \\
    \bottomrule
  \end{tabular}
\end{table*}

% --------------------------------------
\subsection{Varying the Inputs to the Neural Networks}

We also explore changing the set of inputs to the neural networks. For IQ samples, we investigate the following three configurations:
\begin{itemize}
\item ({\bf I}) Use only the input I from the raw IQ samples.
\item ({\bf Q}) Use only the input Q from the raw IQ samples.
\item ({\bf IQ}) Use both I and Q from the raw IQ samples 
\end{itemize}


For the polar representation of IQ samples, we denote the magnitude part as $R=\sqrt{I^2+Q^2}$ and the phase part as $T=\operatorname{arctan} (Q, I)$. As before, we explore three experimental configurations:
\begin{itemize}
\item ({\bf R}) Use only the magnitude R from the polar representation.
\item ({\bf T}) Use only the phase T from the polar representation. input.
\item ({\bf RT}) Use both R and T from the polar representation.
\end{itemize}

For configurations that only provide one input, we zero out the other input.


  % \item The polar representation of IQ samples. Here we denote the magnitude
  %   part of IQ samples as R and the phase part as T. So we have
  %   $R=\sqrt{I^2+Q^2}$ and $T=\operatorname{atan2} (Q, I)$.
  % \item The partial input of IQ samples. The partial input is to set the real
  %   or imaginary part of IQ samples as 0. We can do partial input in both IQ
  %   samples and its polar coordinates form.

%Sometimes the magnitude (R) and phase (T) of IQ samples are more distinguishable
%than the raw IQ. So the results difference under the change of input coordinates
%will show the dominant information of dataset. For the partial input, to zero
%out the real or imaginary part of input will make the CVNN more like RVNN since
%some of the cross items between real part and imaginary part in multiplication
%and convolution operations will be eliminated (see the computational flow in
%Figure \ref{fig:cf_cvnn}, partial input will cause the vanishing of some orange
%and green lines in the figure.), this is also an ablation strategy in some
%sense.


==> abstract-long.tex <==
%Complex numbers are common in science and engineering fields, such as state vectors in Quantum Physics and radio waves in Electrical Engineering. Researchers have demonstrated the effectiveness of neural networks on wireless signals classification. There are also some works on this task by using complex-valued neural networks (CVNNs). But the works to disclose the reason why the complex-valued one is better are still absent.
%
Wireless device identification using deep neural networks has recently received lots of attention due to its potential use in newly emerging applications like spectrum access policy enforcement, unauthorized network access monitoring and control, and anomaly detection. While much of the literature focused on using real-valued convolutional neural networks (RVNNs), some works have shown that complex-valued convolutional neural networks (CVNNs) yield higher device identification and classification accuracy. Although this performance improvement is (intuitively) attributed to the complex representation nature of the sampled RF data (i.e., IQ symbols) used for training and testing these neural networks, no existing work has taken a closer look into analysing such a trend in the context of wireless device identification.
%
In this paper, we took a shot at providing some deep understanding and analysis of the performances of CVNNs in comparison with those of conventional RVNNs. In our study, we used a massive RF fingerprint dataset collected using a testbed consisting of one USRP B210 receiver capturing signals transmitted from 25 LoRa Pycom devices. The dataset covers multiple scenarios, which are specifically designed to allow comprehensive evaluation of CVNNs under different experimental setups.
Our study takes a deep dive into the understanding of the impact (i) of the input representation/type and (ii) of the architectural layer of the neural network. For the input representation impact, we considered the IQ as well as the polar coordinates both partially and fully. For the architectural layer impact, we considered a series of ablation experiments that eliminate a part of the CVNN components (output values or convolutional filter weights) one at a time. Our experiments show that the achievable performance depends on which CVNN architectural layer (low vs. high layer) and component type (output versus filter) are ablated, as well as on the representation form of the input data.

%In this paper, we gave a closer understanding on the benefits of the complex-valued networks on wireless signals. Our results show that CVNNs consistently outperform the real-valued counterpart ($10\% \sim 37\%$) in different datasets of wireless signals. 
%Specifically, from the experiments of the full input and partial input, we observed the CVNNs are able to make better use of the join information of in-phase and quadrature parts of IQ signals. Although the same conclusion cannot be made on polar coordinates form of IQ data, we still can figure out which partial input is dominant in different wireless signals datasets. It's very challenging to transform the CVNN to "equivalent" RVNN, so we design a series ablation experiments which will reduce part of the complex-valued components (output values or the convolutional filter weights of the network layer) and degenerate the CVNN to RVNN as closed as possible. The ablation experiments disclose that the performance has different degrees of loss when removing part of components of CVNN from low-level to high-level layers, and there is slightly different between ablating output and convolutional filter.
